The Best Instruction-Tuning Data are Those That Fit

High-quality supervised fine-tuning (SFT) data are crucial for eliciting strong capabilities from pretrained large language models (LLMs). Typically, instructions are paired with multiple responses sampled from other LLMs, which are often out of the distribution of the target model to be fine-tuned. This, at scale, can lead to diminishing returns and even hurt the models' performance and robustness. We propose **GRAPE**, a novel SFT framework that accounts for the unique characteristics of the target model. For each instruction, it gathers responses from various LLMs and selects the one with the highest probability measured by the target model, indicating that it aligns most closely with the target model's pretrained distribution; it then proceeds with standard SFT training. We first evaluate GRAPE with a controlled experiment, where we sample various solutions for each question in UltraInteract from multiple models and fine-tune commonly used LMs like LLaMA3.1-8B, Mistral-7B, and Qwen2.5-7B on GRAPE-selected data. GRAPE significantly outperforms strong baselines, including distilling from the strongest model with an absolute gain of up to 13.8%, averaged across benchmarks, and training on 3x more data with a maximum performance improvement of 17.3%. GRAPE's strong performance generalizes to realistic settings. We experiment with the post-training data used for Tulu3 and Olmo-2. GRAPE outperforms strong baselines trained on 4.5 times more data by 6.1% and a state-of-the-art data selection approach by 3% on average performance. Remarkably, using 1/3 of the data and half the number of epochs, GRAPE enables LLaMA3.1-8B to surpass the performance of Tulu3-SFT by 3.5%.

==> background-backup.tex <==
\section{Background and Motivation}
\label{sec:motivation}

\paragraph{An analogy from Reinforcement Learning and Preference Learning}
% These observations are supported\hao{this is too strong since below are not sft anymore. `inspired' or `analogous' are more proper} 

The investigation of this work into the distribution match between the pre-trained LM and supervised fine-tuning (SFT) data is inspired by recent findings on policy optimization for LM alignment with RL~\citep{ouyang2022training} and preference learning~\citep{rafailov2023dpo,ethayarajh2024kto}. 
While the importance of matching training data distribution with the  policy has been well noted in both traditional RL~\citep{shi2023offlinereinforcementlearningonpolicy,fujimoto2018offpolicy,kumar2019offpolicy,peng2019offpolicy,wang2021criticregularizedregression,arora2023theory,jiang2016doublyrobustoffpolicyvalue,tang2010importancesampling} and LM settings~\citep{xiong2024iterative}, preference learning algorithms like DPO~\citep{rafailov2023dpo}, IPO~\citep{azar2023ipo} and KTO~\citep{ethayarajh2024kto} first emerged as off-policy algorithms. 
However, subsequent research has highlighted the performance gap between on-policy and off-policy training due to distribution shifts ~\citep{xu2024dposuperiorppollm,tang2024understandingperformancegaponline} and proposed various mitigation strategies ~\citep{zhuang2023bpo,zhou2024wpoenhancingrlhfweighted,zhang2024textbfplumimprovingcodelms,xiong2024iterative,guo2024onlineaifeedback}, showing that training models on data more closely aligned with their policy distribution can significantly improve performance, while failing to do so can yield sub-optimal policies or those that are harder to generalize. 
\paragraph{Hypothesis: Supervised Fine-tuning Benefits From Data That Better Matches Base Distribution}
The base distribution of pre-trained language models---shaped by extensive training on vast and diverse datasets---is inherently robust and generalizable~\citep{brown2020languagemodelsfewshotlearners,saunshi2021mathematicalexplorationlanguagemodels}. Therefore, during supervised fine-tuning phase, the pre-trained distribution should be carefully preserved~\citep{kumar2022finetuningdistortpretrainedfeatures,cohenwang2024askdistributionshiftpretraining,he2023preservingpretrained,yang2024selfdistillationbridgesdistributiongap,ding2023peft}, to best retain the knowledge and capabilities that emerge during pre-training~\citep{zhou2023lima}. 
If the proximity between the pre-trained distribution and the fine-tuning data is not maintained, the limited number of training examples available during SFT, compared to the vast scale of pre-training data, can increase the risk of distribution distortion. This misalignment can lead to issues such as catastrophic forgetting~\citep{aghajanyan2020betterfinetuningreducingrepresentational,yang2024selfdistillationbridgesdistributiongap} and the emergence of spurious correlations~\citep{feldman2021doeslearningrequirememorization}.

The central premise of our work is that by using responses closely aligned to the pre-trained distribution, we can minimize distribution shift during SFT and therefore achieve better data efficiency and stronger performance. 
\paragraph{From On-Policy Alignment To Distribution-Aligned SFT}
\label{sec:on_policy}
We build on principles of on-policy alignment techniques with key distinctions tailored for SFT. 
Yet, given that SFT represents an earlier stage of post-training than RL, sampling responses from the base model itself alone can lead to model collapse, as noted in~\citep{collapse_when_trained_recursive}.
Prior studies have documented similar risks like instability, bias reinforcement, knowledge stagnation, and overfitting~\citep{herel2024collapseselftrainedlanguagemodels,mobahi2020selfdistillationamplifiesregularizationhilbert,allenzhu2023understandingensembleknowledgedistillation,ghosh2024closerlooklimitationsinstruction,dong2025selfboosting,zhang2024forcing}. To address this, we advocate for an approach that stays more in-distribution while delivering effective supervision to the base model. To this end, we propose to gather and select responses from various sources, and select one that is closest to the target model's pretrained distribution, which we name \name.  


==> impact_statement.tex <==
\section*{Impact Statement}
This paper presents work whose goal is to advance the field of Machine Learning.
It investigates fundamental aspects of instruction-tuning of language models and should not have direct societal impacts or implications that should be discussed here specifically, to the best of the authors' knowledge. 

==> intro-backup-jan29.tex <==
% \section{Introduction}
% Instruction tuning has emerged as a pivotal technique for enhancing large language models (LLMs) by aligning them with human intent through task-specific datasets. By fine-tuning on instruction-response pairs, this approach has unlocked remarkable generalization across unseen tasks, making LLMs versatile in real-world applications. 

% Crafting effective instruction-tuning datasets is a non-trivial challenge. Within this domain, up-scaling instruction tuning data by synthesizing more question-answer pairs with language models has been a predominant direction for improving SFT'ed model's performance. But this benefit will not extend forever. Research suggests that models trained on increasingly large collections is likely to stop improving or even starting to decline~\cite{alemohammad2024selfconsuming,gerstgrasser2024iscollapseinevitable,dohmatob2024strongmodelcollapse,shumailov2023curse,Hataya_2023_ICCV, martínez2023combining, martínez2023understanding, bohacek2023nepotistically, briesch2023large} because of the diversity decrease~\cite{padmakumar2024writing, guo2023curious} or distribution distortion~\cite{lebrun2021evaluating}.


% Therefore, effective instruction tuning requires more than expansion of training data size, it also demands a careful introspection into the quality of data, and its utility with respect to a base model~\cite{li2024quantitytoqulality,du2023modsmodelorienteddataselection}. 

% Prior studies have tailored instruction-tuning questions to the characteristics of the base model using approaches like curriculum learning~\cite{zhao2024preliminarystudyintrinsicrelationship,lee2024instructiontuninghumancurriculum,feng2023citinglargelanguagemodels} and targeted instruction expansion~\cite{du2023mods}. While these works emphasize aligning the training data with the model's capacity, or ``talent'', we argue that equal attention should be given to the model's inherent behavioral patterns — its ``tone''. 

% Current datasets often overlooks this aspect and prepares model-agnostic solutions, using solutions generated by more powerful models that could be very exotic to the model one wants to train.

% Moreover, the widely-adopted practice of pairing prompts with multiple responses for data augmentation as done in ~\citet{yu2024metamath,yuan2024eurus} may make the problem of distributional mismatches and spurious correlations even more pronounced, leading to diminishing returns or even performance degradation~\cite{li2024mugglemath,chan2024balancingcosteffectivenesssynthetic,setlur2024rlincorrectsyntheticdata}. 

% These issues highlight the need for targeted response selection strategies that align with the model’s inherent tendencies.

% Inspired by the success of on-policy learning in reinforcement learning and preference alignment~\cite{tajwar2024shoulduse,guo2024onlineaifeedback,setlur2024rlincorrectsyntheticdata,liu2024provablymitigatingoveroptimizationrlhf,chen2024optuneefficientonlinepreference}, we propose a approach to instruction tuning that tailors responses for each model's individual characteristics. Specifically, we hypothesize that responses closer to the base model's current distribution provide more effective training signals, aligning with the model's strengths while reducing the risks of distributional mismatches. By incorporating this distribution-aware perspective into dataset curation, we aim to unlock the untapped potential of aligning instruction data with the base model's unique characteristics.

% To realize this vision, we introduce a novel framework for response selection called \textbf{\name}, which stands for \textbf{G}enerating various candidate responses, \textbf{R}anking them based on their \textbf{A}lignment with the base model's \textbf{P}olicy, and leveraging this ranking to \textbf{E}nhance supervised fine-tuning performance.

% \name first samples solutions from a variety of strong models to from a diverse collection of responses, then ranks these responses based on their likelihood in the base model's distribution and take those that closely aligns with the base model to perform supervised fine-tuning. It ensures a good approximation of the distribution of ``golden'' answers while customizing for each base model to avoid drastic distribution shifts. 

% We validate our approach through comprehensive experiments, demonstrating consistent performance gains across diverse LLM architectures and tasks. Despite its simplicity, the framework achieves substantial improvements in generalization and robustness, offering a scalable solution to the challenges of instruction tuning.

% Through this work, we propose a shift from dataset scaling or feeding the same solutions to every model, to a more tailored, model-aware data curation on the response side. Our findings not only enhance the efficiency of instruction tuning but also pave the way for a deeper understanding of how LLMs interact with their training data, driving the development of more adaptable and high-performing models.
\section{Introduction}

\hao{this first paragraph is perhaps too well-known to have in the intro. i'd drop:}
% Supervised fine-tuning (SFT) has become a cornerstone for unlocking the full potential of large language models (LLMs), enabling them to generalize across diverse, unseen tasks\hao{this is a bit too strong. i'd say eliciting the capabilities of following instruction and solving various tasks}. By fine-tuning on instruction-response pairs, this process bridges the gap between pretrained models and their ability to align with human intent. 
Supervised fine-tuning (SFT) has become a cornerstone for unlocking the full potential of large language models (LLMs). However, crafting high-quality instruction datasets that effectively enhance model capabilities remains a significant challenge.

High-quality, large-scale supervised data is crucial for supervised instruction finetuning (SFT).s 


\hao{I added:
High-quality, large-scale supervised data is crucial for supervised instruction finetuning (SFT).s
}
It has become a well-established approach to collect SFT data by pairing each instruction with responses sampled from multiple LLMs that are usually stronger than the target LLM to be finetuned.\hao{check and cite}
\hao{maybe add a minor note about quality control through, e.g., rejection sampling}
% synthesizing more question-response pairs using stronger LLMs. 
% Recent studies reveal
\hao{this following sent is pretty vague. i;d drop}
While this has shown early promise, recent studies reveal a plateau effect, where performance stagnates or even declines as dataset size increases. 
This phenomenon arises due to issues such as diminishing diversity~\cite{padmakumar2024writing, guo2023curious} and distortion in the data distribution~\cite{lebrun2021evaluating}, which ultimately undermine the base model's performance and robustness~\cite{alemohammad2024selfconsuming, gerstgrasser2024iscollapseinevitable, shumailov2023curse,dohmatob2024strongmodelcollapse,Hataya_2023_ICCV,martínez2023combining,martínez2023understanding,bohacek2023nepotistically,briesch2023large}.



\hao{if we had addressed the comments in the paragraph above (that they are used to scale up the SFT data wjan2hich often results in issues), this would have been a nice transition.
}
Thus, effective instruction tuning often requires more than scaling up the data; 
it often needs  ``tailoring'' the data to the unique characteristics of the target model, which has been studied in the context of curriculum \hao{check}learning~\cite{zhao2024preliminarystudyintrinsicrelationship, lee2024instructiontuninghumancurriculum,feng2023citinglargelanguagemodels,setlur2024rlincorrectsyntheticdata} and \hao{we should clarify how this one differs from \name somewhere:}targeted data curation~\cite{du2023modsmodelorienteddataselection}.
% , aim to adapt instruction tuning to the model's capacity. 
\hao{i didn't get the `talent' vs. `tone' thing below. i doubt it that we actually need this sentence:}
While these approaches consider the model's strengths or ``talent,'' they often overlook the importance of aligning responses with the base model’s inherent behavioral tendencies or ``tone.'' 
Meanwhile, the principle of tailoring the data to the model has been a crucial ingredient for the later phases of LLM development, in the form of on-policy preference learning\hao{cite}, and on-policy/online reinforcement learning (RL)\hao{cite}.
% the importance of ensuring a closer alignment between training data and the behavior policy (of the model to be trained) has been extensively highlighted and utilized in research on reinforcement learning and preference learning
~\cite{xu2024dposuperiorppollm,tajwar2024shoulduse,zhang2024selfexploringlanguagemodelsactive,guo2024onlineaifeedback,liu2024provablymitigatingoveroptimizationrlhf,zhang2024textbfplumimprovingcodelms,miao2024aligningcodellmsdirectpreference,gulcehre2023rest,azar2023generaltheoreticalparadigmunderstand,tang2024understandingperformancegap,zhuang2023bpo,zhou2024wpoenhancingrlhfweighted}.

% This mismatch becomes particularly pronounced when responses are sampled from a very different distribution than the model's base policy, which could lead sub-optimal performance~\cite{li2024mugglemath, chan2024balancingcosteffectivenesssynthetic}. 

% On the other hand 

% To address these challenges, we propose a novel SFT response engineering framework, \name, designed to optimize instruction tuning by tailoring response selection to each base model's distribution. Unlike existing datasets that usually contains one-size-fits-all solutions sampled from one single best model without customization~\cite{yu2024metamath, yuan2024eurus,slimorca,OpenHermes}, \name curates responses that align closely with the base model's pretrained policy. By leveraging a distribution-aware approach, \name mitigates the risks of distribution drift and spurious correlations, while ensuring coverage of optimal solutions.
\hao{i reordered things below}
Inspired by these insights,
we hypothesize that SFT can similarly benefit from aligning data with the model,
the core idea behind \name.
For each instruction, \name {\bf g}athers and selects {\bf r}esponses from various LLMs,
and selects one that is closest to the target model's {\bf p}r\textbf{e}trained distribution.
This is achieved by calculating the perplexity of each response using the target model and selects the one with the lowest perplexity. 
% improved alignment between the base model's distribution and the distribution of the responses in the training data. 
% We propose \name which {\bf g}athers diverse {\bf r}esponses for each instruction from various sources and score them based on how well they {\bf a}lign with the base LLM’s {\bf p}r\textbf{e}trained distribution. 
% Thus, \name offers a surprisingly simple and efficient approach: it calculates the perplexity of each candidate response for a given instruction using the base model and selects the response with the lowest perplexity. 
Unlike existing datasets that usually contains one-size-fits-all responses for each instruction without customization~\cite{yu2024metamath, yuan2024eurus,slimorca,OpenHermes}, \name curates model-dependent SFT datasets that better mitigates the risks of distribution shift \hao{why does it fix the following issues?:} and spurious correlations, while posing minimum overhead for dataset collation. 

% By leveraging a distribution-aware approach, \name mitigates the risks of distribution drift and spurious correlations, while ensuring coverage of optimal solutions.

% Specifically, \name follows a two-step process: (1) collecting diverse responses from various strong LLMs to build a comprehensive candidate pool, and (2) ranking and selecting responses based on their likelihood under the base model’s distribution. This approach balances diversity and alignment, approximating the ``golden'' distribution while customizing the training data for the base model’s unique tendencies.

\name is simple and effective, and adds little overhead to the SFT process.
To \name's advantage, many existing datasets share overlapping instructions but contain different high-quality responses. One can therefore directly select, for each model, the best fit(s) among the off-the-shelf responses without needing to produce new responses. 
We first validate the  extensive controlled experiments on chain-of-thought reasoning scenario and demonstrate 
Through extensive experiments on stepwise reasoning tasks, we demonstrate the efficacy of \name. Notably, models fine-tuned with \name-selected responses outperform those trained on 3-times datasets and responses from the strongest models among all. This underscores the critical role of tailored data curation in optimizing SFT performance.

\todo{Talk about data selection set-up}

\hao{don't think we need this:}
We advocate for a model-aware approach to instruction tuning that tailors response selection to the base model. By shifting the focus from dataset scaling to strategic data alignment, \name advances the understanding of LLM training dynamics and sets a new benchmark for scalable, high-performance instruction tuning.


==> proof.tex <==
\section{Appendix: Detailed Math Proofs}

\subsection{Preliminaries}

We consider discrete distributions over a finite set of responses $\mathcal{R}$. 
For distributions $p$ and $q$ on $\mathcal{R}$, recall the Kullback-Leibler (KL) divergence:
\[
D_{\mathrm{KL}}(p \,\|\, q) 
\;=\; 
\sum_{r \in \mathcal{R}} p(r)\,\log\!\Bigl(\tfrac{p(r)}{q(r)}\Bigr).
\]
KL divergence is always non-negative and $D_{\mathrm{KL}}(p\|q) = 0$ iff $p = q$ (almost everywhere).

\subsection{Theorem~1: Policy-Guided Selection Minimizes KL}

\begin{theorem}
\label{thm:kl-min-selection}
Let $\tilde{\mathcal{R}}_i$ be a candidate pool of valid responses. Suppose we want to select a subset of size $K$ and assign a probability distribution $\tilde{\pi}$ on that subset. Our objective is to \emph{minimize} $D_{\mathrm{KL}}(\tilde{\pi} \,\|\, \pi_{\theta_0})$. 

Then the solution is:
\begin{itemize}
    \item Choose the top-$K$ responses $\mathcal{R}_i^{\theta_0}$ under $\pi_{\theta_0}$ (i.e.\ those $r$ for which $\pi_{\theta_0}(r)$ is largest).
    \item Set $\tilde{\pi}(r) \propto \pi_{\theta_0}(r)$ for $r \in \mathcal{R}_i^{\theta_0}$.
\end{itemize}

For any other distribution $\tilde{\pi}_{\mathrm{rand}}$ supported on some subset of size $K$, 
\[
D_{\mathrm{KL}}\bigl(\hat{\pi}_{\theta_0}\,\big\|\,\pi_{\theta_0}\bigr) 
\;\le\; 
D_{\mathrm{KL}}\bigl(\tilde{\pi}_{\mathrm{rand}}\,\big\|\,\pi_{\theta_0}\bigr).
\]
\end{theorem}

\begin{proof}
\textbf{Step 1: Fix a $K$-element support and solve for $\tilde{\pi}$.}\\
Fix any subset $S \subseteq \tilde{\mathcal{R}}_i$ of size $K$. Among distributions $\tilde{\pi}$ with $\mathrm{Supp}(\tilde{\pi}) = S$, we want to solve:
\[
\min_{\tilde{\pi}:\,\mathrm{Supp}(\tilde{\pi})=S} \; 
D_{\mathrm{KL}}\bigl(\tilde{\pi}\,\|\,\pi_{\theta_0}\bigr).
\]
Expand the KL:
\[
D_{\mathrm{KL}}(\tilde{\pi}\,\|\,\pi_{\theta_0}) 
= \sum_{r \in S} \tilde{\pi}(r)\,\log\!\Bigl(\tfrac{\tilde{\pi}(r)}{\pi_{\theta_0}(r)}\Bigr).
\]
Use Lagrange multipliers or note that for fixed support $S$, this KL is minimized by setting 
\[
\tilde{\pi}(r) \;=\; \frac{\pi_{\theta_0}(r)}{\sum_{r'\in S}\pi_{\theta_0}(r')}, 
\quad r \in S.
\]
Thus the minimizer is precisely the renormalized distribution of $\pi_{\theta_0}$ on $S$.

\noindent
\textbf{Step 2: Find the best $K$-element subset.}\\
Now we want to choose $S$ of size $K$ to minimize $D_{\mathrm{KL}}(\tilde{\pi}\,\|\,\pi_{\theta_0})$. 
Given Step~1, the minimal KL with support $S$ is
\[
\sum_{r \in S} \frac{\pi_{\theta_0}(r)}{\sum_{r'\in S}\pi_{\theta_0}(r')} 
   \,\log\!\Bigl(\tfrac{\pi_{\theta_0}(r)/Z_S}{\pi_{\theta_0}(r)}\Bigr),
\]
where $Z_S = \sum_{r'\in S} \pi_{\theta_0}(r')$.  Simplify the logarithm:
\[
\log\!\Bigl(\tfrac{\pi_{\theta_0}(r)/Z_S}{\pi_{\theta_0}(r)}\Bigr) 
= \log\!\Bigl(\tfrac{1}{Z_S}\Bigr) 
= -\log(Z_S).
\]
So
\[
D_{\mathrm{KL}}(\tilde{\pi}\,\|\,\pi_{\theta_0}) 
= \sum_{r \in S} \frac{\pi_{\theta_0}(r)}{Z_S}\,\bigl(-\log Z_S \bigr) 
= -\log Z_S \;\sum_{r \in S} \frac{\pi_{\theta_0}(r)}{Z_S}.
\]
But $\sum_{r \in S} \frac{\pi_{\theta_0}(r)}{Z_S} = 1$. Hence
\[
D_{\mathrm{KL}}(\tilde{\pi}\,\|\,\pi_{\theta_0}) = -\log Z_S.
\]
Because $\pi_{\theta_0}(r)\ge 0$, we have $Z_S = \sum_{r\in S} \pi_{\theta_0}(r)$. Minimizing $-\log Z_S$ is equivalent to \emph{maximizing} $Z_S$ over all $K$-element subsets $S \subseteq \tilde{\mathcal{R}}_i$. This maximum is achieved by picking the $K$ elements with the largest values of $\pi_{\theta_0}(r)$, i.e.\ the top-$K$ responses. 

Thus the distribution $\hat{\pi}_{\theta_0}$ that re-normalizes $\pi_{\theta_0}$ onto its top-$K$ support uniquely minimizes the KL.

\noindent
\textbf{Step 3: Compare to any random subset.}\\
A random subset $\mathcal{R}_i^{(\mathrm{rand})}$ supported on $K$ elements that are not necessarily the top-$K$ by $\pi_{\theta_0}$ results in $Z_S$ that is strictly smaller (unless it accidentally picks exactly those top-$K$). Thus $-\log Z_S$ is strictly larger, giving a strictly larger KL. This proves the theorem.
\end{proof}


\subsection{Theorem~2: Closer to the Golden Distribution}

\begin{theorem}
\label{thm:closer-golden}
Let $\hat{\pi}_{\theta_0}$ be the distribution over $\tilde{\mathcal{R}}_i$ formed by selecting top-$K$ valid responses and renormalizing $\pi_{\theta_0}$. Suppose $\tilde{\mathcal{R}}_i$ is drawn from a mixture $\pi_{\mathcal{C}}^{(\cup)}$ that is itself closer to $\pi^*$ than $\pi_{\theta_0}$. Then:
\[
D_{\mathrm{KL}}\Bigl(\hat{\pi}_{\theta_0}\,\Big\|\,\pi^*\Bigr) 
\;<\; 
D_{\mathrm{KL}}\Bigl(\pi_{\theta_0}\,\Big\|\,\pi^*\Bigr).
\]
\end{theorem}

\begin{proof}
\textbf{Step 1: Restricting support to valid responses.}\\
Since $\tilde{\mathcal{R}}_i$ is sampled from policies $\{\pi_{\mathcal{C}}^{(m)}\}$ that presumably place high probability on valid or near-correct solutions (closer to $\pi^*$), the set $\tilde{\mathcal{R}}_i$ excludes many low-quality responses that $\pi_{\theta_0}$ might have supported originally.

\noindent
\textbf{Step 2: Construct $\hat{\pi}_{\theta_0}$.}\\
Within $\tilde{\mathcal{R}}_i$, we keep the top-$K$ responses under $\pi_{\theta_0}$. By removing responses outside $\tilde{\mathcal{R}}_i$ (many of which might be misaligned or invalid), $\hat{\pi}_{\theta_0}$ effectively ``truncates'' the mass of $\pi_{\theta_0}$ to presumably better responses in $\tilde{\mathcal{R}}_i$.

\noindent
\textbf{Step 3: KL comparison.}\\
Write the KL divergences:
\[
D_{\mathrm{KL}}\bigl(\hat{\pi}_{\theta_0}\,\|\,\pi^*\bigr) 
= \sum_{r \in \mathcal{R}_i^{\theta_0}} \hat{\pi}_{\theta_0}(r)\,\log\!\Bigl(\tfrac{\hat{\pi}_{\theta_0}(r)}{\pi^*(r)}\Bigr).
\]
Meanwhile,
\[
D_{\mathrm{KL}}\bigl(\pi_{\theta_0}\,\|\,\pi^*\bigr) 
= \sum_{r \in \mathcal{R}} \pi_{\theta_0}(r)\,\log\!\Bigl(\tfrac{\pi_{\theta_0}(r)}{\pi^*(r)}\Bigr).
\]
Because $\hat{\pi}_{\theta_0}$ zeroes out probability on responses not in $\mathcal{R}_i^{\theta_0}$ and reweights on valid or good responses, it systematically removes the contributions to KL from any bad out-of-support $r$ that $\pi^*$ also places near-zero mass on. 
Hence $D_{\mathrm{KL}}(\hat{\pi}_{\theta_0}\,\|\,\pi^*)$ is \emph{strictly less} than $D_{\mathrm{KL}}(\pi_{\theta_0}\,\|\,\pi^*)$ (unless $\pi_{\theta_0}$ was already perfectly aligned). 
\end{proof}


==> tables/olmo.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[h]
\small
\centering
\begin{tabular}{llcccccc}
\hline
 &
   &
  \textbf{BBH} &
  \textbf{MMLU} &
  \textbf{IFEval} &
  \textbf{GSM-Plus} &
  \textbf{MATH} &
  \textbf{LeetCode} \\ \hline
 &
  \cellcolor[HTML]{ECF4FF}\textbf{\name-Selected} &
  \cellcolor[HTML]{ECF4FF}62.3 &
  \cellcolor[HTML]{ECF4FF}58.0 &
  \cellcolor[HTML]{ECF4FF}59.0 &
  \cellcolor[HTML]{ECF4FF}45.3 &
  \cellcolor[HTML]{ECF4FF}22.5 &
  \cellcolor[HTML]{ECF4FF}15.6 \\
\multirow{-2}{*}{\textsc{Mistral-v0.3-7B}} &
  \textbf{Highest Loss} &
  57.2 &
  56.0 &
  54.1 &
  37.0 &
  14.8 &
  10.0 \\ \hline
 &
  \cellcolor[HTML]{ECF4FF}\textbf{\name-Selected} &
  \cellcolor[HTML]{ECF4FF}73.4 &
  \cellcolor[HTML]{ECF4FF}73.3 &
  \cellcolor[HTML]{ECF4FF}68.1 &
  \cellcolor[HTML]{ECF4FF}64.0 &
  \cellcolor[HTML]{ECF4FF}49.9 &
  \cellcolor[HTML]{ECF4FF}47.2 \\
\multirow{-2}{*}{\textsc{Qwen2.5-7B}} &
  \textbf{Highest Loss} &
  72.4 &
  72.8 &
  62.7 &
  63.4 &
  47.7 &
  42.8 \\ \hline
\end{tabular}
\caption{Experiment on Olmo dataset.}
\label{tab:olmo}
\end{table*}

==> tables/tulu.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[h]
\small
 \centering
\begin{tabular}{llcccccc}
\hline
 &
   &
  \textbf{BBH} &
  \textbf{MMLU} &
  \textbf{IFEval} &
  \textbf{GSM-Plus} &
  \textbf{MATH} &
  \textbf{LeetCode} \\ \hline
 &
  \cellcolor[HTML]{ECF4FF}\textbf{\name-Selected} &
  \cellcolor[HTML]{ECF4FF}62.1 &
  \cellcolor[HTML]{ECF4FF}57.3 &
  \cellcolor[HTML]{ECF4FF}50.1 &
  \cellcolor[HTML]{ECF4FF}47.8 &
  \cellcolor[HTML]{ECF4FF}21.1 &
  \cellcolor[HTML]{ECF4FF}12.8 \\
\multirow{-2}{*}{\textsc{Mistral-v0.3-7B}} &
  \textbf{Not-Selected} &
  59.5 &
  56.0 &
  48.6 &
  46 &
  20 &
  11.7 \\ \hline
 &
  \cellcolor[HTML]{ECF4FF}\textbf{\name-Selected} &
  \cellcolor[HTML]{ECF4FF}72.2 &
  \cellcolor[HTML]{ECF4FF}73.2 &
  \cellcolor[HTML]{ECF4FF}60 &
  \cellcolor[HTML]{ECF4FF}64.6 &
  \cellcolor[HTML]{ECF4FF}65.2 &
  \cellcolor[HTML]{ECF4FF}43.8 \\
\multirow{-2}{*}{\textsc{Qwen2.5-7B}} &
  \textbf{Not-Selected} &
  72.0 &
  72.0 &
  53.4 &
  63.4 &
  64.0 &
  42.3 \\ \hline
\end{tabular}
\caption{Experiment on Tulu dataset.}
\label{tab:tulu}
\end{table*}
